Reverse Engineering of Generative Models: Inferring Model Hyperparameters from Generated Images

State-of-the-art (SOTA) Generative Models (GMs) can synthesize photo-realistic images that are hard for humans to distinguish from genuine photos. Identifying and understanding manipulated media are crucial to mitigate the social concerns on the potential misuse of GMs. We propose to perform reverse engineering of GMs to infer model hyperparameters from the images generated by these models. We define a novel problem, ``model parsing", as estimating GM network architectures and training loss functions by examining their generated images -- a task seemingly impossible for human beings. To tackle this problem, we propose a framework with two components: a Fingerprint Estimation Network (FEN), which estimates a GM fingerprint from a generated image by training with four constraints to encourage the fingerprint to have desired properties, and a Parsing Network (PN), which predicts network architecture and loss functions from the estimated fingerprints. To evaluate our approach, we collect a fake image dataset with $100$K images generated by $116$ different GMs. Extensive experiments show encouraging results in parsing the hyperparameters of the unseen models. Finally, our fingerprint estimation can be leveraged for deepfake detection and image attribution, as we show by reporting SOTA results on both the deepfake detection (Celeb-DF) and image attribution benchmarks.

==> con_mat.tex <==
\begin{figure*}[t]
\captionsetup[sub]{font=scriptsize,labelfont={sf}}
\renewcommand{\thesubfigure}{\arabic{subfigure}}
\centering

\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/n1.png}
\caption{norm. type}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/n2.png}
\caption{nonlin. type in blocks}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/n3.png}
\caption{nonlin. type in last ly.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/n4.png}
\caption{up-samp. type}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/n5.png}
\caption{skip conn}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/n6.png}
\caption{down-samp}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L1.png}
\caption{Pixel}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L2.png}
\caption{Discriminator}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L3.png}
\caption{Classification}
\end{subfigure}\!


\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L91.png}
\caption{L1}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L92.png}
\caption{L2}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L93.png}
\caption{MSE}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L94.png}
\caption{MMD}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L95.png}
\caption{Adversarial.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L96.png}
\caption{WGAN.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L97.png}
\caption{KL}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/wce/L98.png}
\caption{CE}
\end{subfigure}\!

\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/n1.png}
\caption{norm. type}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/n2.png}
\caption{nonlin. type in blocks}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/n3.png}
\caption{nonlin. type in last ly.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/n4.png}
\caption{up-samp. type}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/n5.png}
\caption{skip conn}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/n6.png}
\caption{down-samp}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L1.png}
\caption{Pixel}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L2.png}
\caption{Discriminator}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L3.png}
\caption{Classification}
\end{subfigure}\!


\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L91.png}
\caption{L1}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L92.png}
\caption{L2}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L93.png}
\caption{MSE}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L94.png}
\caption{MMD}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L95.png}
\caption{Adversarial.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L96.png}
\caption{WGAN.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L97.png}
\caption{KL}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/confusion_matrix/sce/L98.png}
\caption{CE}
\end{subfigure}\!
\\
\vspace{2mm}
\caption{Confusion matrix for every discrete parameter in network architecture and every parameter in coarse/fine level loss function. $1$-$17$: Weighted cross-entropy and $18$-$34$: Standard cross entropy. }
\label{fig:con_mat}
\end{figure*}



\iffalse

\resizebox{\linewidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/n2.png}\!
\includegraphics[]{figures/confusion_matrix/wce/n3.png}\!
\includegraphics[]{figures/confusion_matrix/wce/n4.png}\!
\includegraphics[]{figures/confusion_matrix/wce/n5.png}\!
\includegraphics[]{figures/confusion_matrix/wce/n6.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L1.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L2.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L3.png}\!}
\resizebox{0.89\linewidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/L91.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L92.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L93.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L94.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L95.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L96.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L97.png}\!
\includegraphics[]{figures/confusion_matrix/wce/L98.png}\!
}
\resizebox{\linewidth}{!}{
\includegraphics[]{figures/confusion_matrix/sce/n1.png}\!
\includegraphics[]{figures/confusion_matrix/sce/n2.png}\!
\includegraphics[]{figures/confusion_matrix/sce/n3.png}\!
\includegraphics[]{figures/confusion_matrix/sce/n4.png}\!
\includegraphics[]{figures/confusion_matrix/sce/n5.png}\!
\includegraphics[]{figures/confusion_matrix/sce/n6.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L1.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L2.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L3.png}\!}
\resizebox{0.89\linewidth}{!}{
\includegraphics[]{figures/confusion_matrix/sce/L91.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L92.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L93.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L94.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L95.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L96.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L97.png}\!
\includegraphics[]{figures/confusion_matrix/sce/L98.png}\!
}


\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/n1.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/n1.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/n3.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/n4.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/n5.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/n6.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/L1.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/L2.png}\!
}
\resizebox{0.25\columnwidth}{!}{
\includegraphics[]{figures/confusion_matrix/wce/L3.png}\!
}
\fi

==> heatmap_fig_loss.tex <==
\begin{figure*}[t]

\resizebox{0.8\linewidth}{!}{
\includegraphics[]{figures/heatmap/L31.png}\quad
\includegraphics[]{figures/heatmap/L32.png}\quad
\includegraphics[]{figures/heatmap/L33.png}\quad
\includegraphics[]{figures/heatmap/L91.png}\quad
\includegraphics[]{figures/heatmap/L92.png}\quad
\includegraphics[]{figures/heatmap/L93.png}
}

\resizebox{\linewidth}{!}{
\includegraphics[]{figures/heatmap/L94.png}\quad
\includegraphics[]{figures/heatmap/L95.png}\quad
\includegraphics[]{figures/heatmap/L96.png}\quad
\includegraphics[]{figures/heatmap/L97.png}\quad
\includegraphics[]{figures/heatmap/L98.png}\quad


}

\caption{Feature heatmap for each feature in loss type predicted feature vector.}
\label{fig:heatmap_loss}
%\vspace{-3mm}
\end{figure*}

==> heatmap_fig_net.tex <==
\begin{figure*}[t]
\captionsetup[sub]{font=scriptsize,labelfont={sf}}
\renewcommand{\thesubfigure}{\arabic{subfigure}}
\centering

\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n11.png}
\caption{norm. type}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n12.png}
\caption{nonlin. type in blocks}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n13.png}
\caption{nonlin. type in last ly.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n14.png}
\caption{up-samp. type}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n15.png}
\caption{skip conn}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n16.png}
\caption{down-samp}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n17.png}
\caption{Pixel}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n18.png}
\caption{Discriminator}
\end{subfigure}\!


\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n19.png}
\caption{L1}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n2.png}
\caption{L2}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n3.png}
\caption{MSE}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n4.png}
\caption{MMD}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n5.png}
\caption{Adversarial.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n6.png}
\caption{WGAN.}
\end{subfigure}\!
\begin{subfigure}{0.11\textwidth}
\includegraphics[width=\linewidth]{figures/heatmap/n7.png}
\caption{KL}
\end{subfigure}\!


\vspace{2mm}
\caption{Confusion matrix for every discrete parameter in network architecture and every parameter in coarse/fine level loss function. $1$-$17$: Weighted cross-entropy and $18$-$34$: Standard cross entropy. }
\label{fig:con_mat}
\end{figure*}





\iffalse
\begin{figure*}[t]
\begin{center}
\resizebox{\linewidth}{!}{
%\includegraphics[]{figures/heatmap/n0.png}\quad
%\includegraphics[]{figures/heatmap/n1.png}\quad
\includegraphics[]{figures/heatmap/n11.png}\quad
\includegraphics[]{figures/heatmap/n12.png}\quad
\includegraphics[]{figures/heatmap/n13.png}\quad
\includegraphics[]{figures/heatmap/n14.png}\quad
\includegraphics[]{figures/heatmap/n15.png}
}

\resizebox{\linewidth}{!}{
%\includegraphics[]{figures/heatmap/n0.png}\quad
%\includegraphics[]{figures/heatmap/n1.png}\quad
\includegraphics[]{figures/heatmap/n16.png}\quad
\includegraphics[]{figures/heatmap/n17.png}\quad
\includegraphics[]{figures/heatmap/n18.png}\quad
\includegraphics[]{figures/heatmap/n19.png}\quad
\includegraphics[]{figures/heatmap/n2.png}
}

\resizebox{\linewidth}{!}{
%\includegraphics[]{figures/heatmap/n0.png}\quad
%\includegraphics[]{figures/heatmap/n1.png}\quad
\includegraphics[]{figures/heatmap/n3.png}\quad
\includegraphics[]{figures/heatmap/n4.png}\quad
\includegraphics[]{figures/heatmap/n5.png}\quad
\includegraphics[]{figures/heatmap/n6.png}\quad
\includegraphics[]{figures/heatmap/n7.png}
}
\caption{\small Feature heatmap for each feature in network architecture predicted feature vector.}
\label{fig:heatmap_net}
\end{center}
%\vspace{-3mm}
\end{figure*}
\fi


==> tab_classify_gm.tex <==
\begin{table}[t!]
\begin{center}
\caption{For each unseen test GM, we find the closest GM within the training set by comparing the predicted hyperparameters with the ground truth hyperparameters of training GMs.}
\begin{adjustbox}{width=1\columnwidth}
\label{tab:clasify_GM}
\begin{tabular}{|c|c|c|c|} \hline
Test GM & Closest GM & Test GM & Closest GM\\\hline
STANDARD\_VAE & BETA\_B\_VAE & STYLEGAN2 & PGAN\\
FACTOR\_VAE & BETA\_B\_VAE & BEGAN & SNGAN\\
BETA\_H\_VAE & BETA\_TC\_VAE & STYLEGAN & PGAN\\
BETA\_TC\_VAE & BETA\_B\_VAE & STGAN & CRAMERGAN\\
DCGAN & MAGAN & SAGAN & MAGAN\\
MMDGAN & BEGAN & FFGAN & STARGAN \\
MRGAN & CRAMERGAN & PGAN & STYLEGAN\\
CRAMERGAN & SNGAN & COCOGAN & STYLEGAN2 \\
SNGAN & CRAMERGAN & DFCVAE & CRAMERGAN \\
MAGAN & BEGAN & DRGAN & COCOGAN\\
BETA\_B\_VAE & DCGAN & TPGAN & CRAMERGAN\\
VAEGAN & PGAN & FSGAN & MAGAN\\ 
OCFGAN & SNGAN & SEAN & STYLEGAN \\
STARGAN & MAGAN & STARGAN2 & CRAMERGAN\\\hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}

==> tab_net_gt2.tex <==
\begin{table}[t]

\begin{center}
\caption{Feature value for different labels of multi-class and binary features.}
\tiny
\label{tab:net_gt_labels}
\begin{adjustbox}{width=1\columnwidth}
\begin{tabular}{|c|c|c|}\hline
Feature & Label & Value \\\hline
\multirow{4}{*}{F$10$}& $0$ & Batch Normalization \\
& $1$ & Instance Normalization \\
& $2$ & Adaptive Instance Normalization \\
& $3$ & No Normalization \\\hline
\multirow{4}{*}{F$11$}& $0$ & ReLU \\
& $1$ & Tanh \\
& $2$ & Leaky\_ReLU  \\
& $3$ & Sigmoid  \\\hline
\multirow{4}{*}{F$12$}& $0$ & ELU \\
& $1$ & ReLU \\
& $2$ & Leaky\_ReLU  \\
& $3$ & Sigmoid  \\\hline
\multirow{2}{*}{F$13$}& $0$ & Nearest Neighbour \\
& $1$ & Deconvolution \\\hline
\multirow{2}{*}{F$14$ and F$15$}& $0$ & Feature used \\
& $1$ & Feature not used \\\hline
    
\end{tabular}
\end{adjustbox}
\end{center}
\end{table}
